Exploring the Impact of Synthetic Data for Aerial-view Human Detection

Aerial-view human detection has a large demand for large-scale data to capture more diverse human appearances compared to ground-view human detection. Therefore, synthetic data can be a good resource to expand data, but the domain gap with real-world data is the biggest obstacle to its use in training. As a common solution to deal with the domain gap, the sim2real transformation is used, and its quality is affected by three factors: i) the real data serving as a reference when calculating the domain gap, ii) the synthetic data chosen to avoid the transformation quality degradation, and iii) the synthetic data pool from which the synthetic data is selected. In this paper, we investigate the impact of these factors on maximizing the effectiveness of synthetic data in training in terms of improving learning performance and acquiring domain generalization ability--two main benefits expected of using synthetic data. As an evaluation metric for the second benefit, we introduce a method for measuring the distribution gap between two datasets, which is derived as the normalized sum of the Mahalanobis distances of all test data. As a result, we have discovered several important findings that have never been investigated or have been used previously without accurate understanding. We expect that these findings can break the current trend of either naively using or being hesitant to use synthetic data in machine learning due to the lack of understanding, leading to more appropriate use in future research.

==> Contents/ECCV2024/acknowledgement.tex <==


\noindent{\bf Acknowledgements.} This research was sponsored by the Defense Threat Reduction Agency (DTRA) Contract Number: A2205097021023559. This research was also supported in part by the U.S. Army Research Office and Army Research Laboratory under Award No. W911NF2110258.

==> Contents/ECCV2024/results.tex <==
\section{Results and Analysis}
\label{sec:analysis}

\subsection{A Study on the Impact of Real Data}

For the first study, we explore the scalability behavior of real data regarding the two impacts of using synthetic data in training: i) increasing detection accuracy and ii) reducing the distribution gaps. Specifically, these two aspects are compared among four cases using real data with different quantities (\ie, 20, 50, 100, and 200).\smallskip


\begin{figure}[t]
\centering
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_real_same_domain.pdf}
\vspace{-0.3cm}
\caption{}
\label{fig:num_real_same_domain}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_real_cross_domain.pdf}
\vspace{-0.3cm}
\caption{}
\label{fig:num_real_cross_domain}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ratio_real_cross_domain.pdf}
\vspace{-0.3cm}
\caption{}
\label{fig:num_real_ratio}
\end{subfigure}
\vspace{-0.3cm}
\caption{{\bf Accuracy with the size of real dataset.} (b) and (c) show the accuracy when synthetic images are used in training.}
\label{fig:scaling_behavior_of_realimg}
\end{figure}

\noindent{\bf Analysis in terms of accuracy.} In same-domain tasks (Fig.~\ref{fig:num_real_same_domain}), detection accuracy unsurprisingly increased proportionally with the size of the real dataset, regardless of whether or not synthetic data is used. The use of synthetic data consistently increases accuracy irrespective of the size of the real data set. Interestingly, adopting a larger real dataset yields better accuracy even in most cross-domain tasks (Fig.~\ref{fig:num_real_cross_domain}). These trends indicate that it is essential to use synthetic data with real data, including cross-domain tasks.

Using a large number of real images (\ie, 200), on the other hand, results in little increase or adversely affects accuracy compared to using fewer images. The rationale behind this notable observation can be accounted for with Fig.~\ref{fig:num_real_ratio}, which illustrates the accuracy ratio of a cross-domain task to a same-domain task. Here, the two tasks use different training sets (for the cross-domain task, we use VisDrone as the training set.) but are evaluated on the same test set. When the number of real images is small, the cross-domain presents similar or better accuracy than the same-domain. However, the effectiveness of the cross-domain continues to decrease as the number of real images increases. 

These analyses strongly indicate that \emph{synthetic data is effective in both same-domain and cross-domain tasks, particularly the impact of synthetic images is more significant when the amount of real data is small and then it continues to diminish as the amount of real data increases}. These findings fully confirm that synthetic data can greatly enhance learning in the data scarcity realm, where real data are hard to obtain if adequately integrated into learning.\smallskip

\input{Tables/distributon_gap_full}


\noindent{\bf Analysis in terms of distribution gaps.} Table~\ref{tab:distribution_gap} provides distribution gaps for the various test sets with and without synthetic data in a cross-domain setup. It is observed that for some cases, the use of synthetic data (`all' in the Table) unexpectedly increases the distribution gap compared to the cases without synthetic data. On the other hand, the distribution gap over half of the test images located closer to the reference dataset in terms of the Mahalanobis distance (`50\%' in the Table) decreased as expected when synthetic data is added.

To investigate the change in the distribution gap in detail, we compare histograms representing the number of test images with respect to the Mahalanobis {% tex broke the page here!!!!
\parfillskip=0pt
\parskip=0pt
\par}

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\begin{subfigure}{.49\linewidth}
\includegraphics[width=\linewidth,trim=5mm 0mm 10mm 0mm,clip]{Figures/hist_oku_vis50.pdf}
\caption{}
\label{fig:histogram}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
\includegraphics[width=\linewidth,trim=5mm 0mm 10mm 0mm,clip]{Figures/scatter_oku_vis50.pdf}
\caption{}
\label{fig:scatter}
\end{subfigure}
\vspace{-0.7cm}
\caption{{\bf Change in distribution gap when synthetic images are used} for each image of the Okutama-Action dataset under the Vis-50 setup.}
\end{wrapfigure} 

\noindent distance with and without synthetic data (Fig.~\ref{fig:histogram}). Including synthetic data effectively reduces the Mahalanobis distance for most of the test images, yet the number of outliers with extremely large Mahalanobis distances also increases. We also compare how the distribution of test images with respect to detection scores \vs.~Mahalanobis distances differ depending on whether synthetic data is included or not (Fig.~\ref{fig:scatter}). When using synthetic data in training, a majority of test images come with high detection confidence and small Mahalanobis distances, contributing to a detection accuracy increase. However, the test images with large Mahalanobis distances and low detection confidence also appear more frequently. The analysis indicates that \emph{a majority of synthetic data serves to improve the detector's ability for most test images in general with some exceptions of outlier images in a cross-domain setup}.


\subsection{A Study on the Impact of Synthetic Data}

For the second study, we explored the scalability behavior of synthetic data on the two impacts of using the synthetic data in training, mentioned in the first study. Specifically, we compare five cases with no synthetic images, 100, 500, 1000, and 2000 synthetic images in training in terms of the accuracy and distribution gap.\smallskip

\begin{figure}[t]
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_same_domain_vis_20.pdf}
\label{fig:num_synth_same_domain_vis_20}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_same_domain_vis_50.pdf}
\label{fig:num_synth_same_domain_vis_50}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_same_domain_vis_100.pdf}
\label{fig:num_synth_same_domain_vis_100}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_same_domain_vis_200.pdf}
\label{fig:num_synth_same_domain_vis_200}
\end{subfigure}
\\
\begin{subfigure}{0.24\linewidth}
\vspace{-0.4cm}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_cross_domain_vis_20.pdf}
\label{fig:num_synth_cross_domain_vis_20}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\vspace{-0.4cm}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_cross_domain_vis_50.pdf}
\label{fig:num_synth_cross_domain_vis_50}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\vspace{-0.4cm}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_cross_domain_vis_100.pdf}
\label{fig:num_synth_cross_domain_vis_100}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\vspace{-0.4cm}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/ap_synth_cross_domain_vis_200.pdf}
\label{fig:num_synth_cross_domain_vis_200}
\end{subfigure}
\vspace{-0.6cm}
\caption{{\bf Accuracy with the size of the synthetic dataset.} Plots in the top and bottom rows show APs in same-domain and cross-domain tasks, respectively.}
\label{fig:scaling_behavior_of_synthimg}
\end{figure}

\noindent{\bf Analysis in terms of accuracy.} In this study, as PTL, our standard method of using synthetic images in training, gradually increases the number of synthetic images as training progresses, we investigate the scaling behavior of synthetic data by comparing models at different training checkpoints. To exclude the potential methodological influence of PTL in this general investigation, we also consider a random selection method, which randomly selects the same number of synthetic images as those used in PTL for training after applying the sim2real transformation.

In Fig.~\ref{fig:scaling_behavior_of_synthimg}, two notable observations can be found regarding accuracy: i) in all setups, including same-domain and cross-domain, regardless of the method for synthetic data integration, the accuracy continues to increase while the rate of accuracy increase decreases as more synthetic images are used in training, and ii) as more real images are used in training, the checkpoint where the increase in accuracy rapidly diminishes usually occurs when a relatively large number of synthetic images are used. These observations indicate that \emph{the impact of synthetic data continues to decrease as more synthetic images are included, but the capacity to use more synthetic data without sacrificing accuracy is expanded as more real data is used}.\smallskip

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-0.8cm}
\begin{subfigure}{0.47\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/scatter_oku_vis50_PTL_v2.pdf}
\label{fig:scatter_PTL}
\end{subfigure}
\hfill
\begin{subfigure}{0.47\linewidth}
\includegraphics[trim=10mm 0mm 10mm 0mm,clip,width=\linewidth]{Figures/scatter_oku_vis50_random_v2.pdf}
\label{fig:scatter_random}
\end{subfigure}
\vspace{-0.5cm}
\caption{{\bf Detection accuracy-distribution gap scatter plot with various numbers of synthetic images.} The left and right plots are made with PTL and a random selection, respectively, using the Okutama-Action dataset under the Vis-50 setup. Darker dots represent test data when using more synthetic images for training.}
\label{fig:scatter_of_synthimg}
\vspace{-0.6cm}
\end{wrapfigure}


\noindent{\bf Analysis in terms of distribution gaps.} In Table~\ref{tab:distribution_gap_with_various_synthetic_images} that shows the scalability behavior of synthetic data with respect to the distribution gap, it is observed that the distribution gap mostly continues to decrease while the rate of change also decreases as more synthetic images are used in training. This is aligned to that of the previous analysis regarding accuracy.

In Fig~\ref{fig:scatter_of_synthimg}, we can figure out how the distribution of test images for the detection score and Mahalanobis distance changed with the number of synthetic images used in training. Two notable observations are presented in the scatter plots: i) samples with high detection score ($>$0.2) appear more often as more synthetic images are used, and ii) samples with large Mahalanobis distance also appear more frequently when using a very large number of synthetic images (\ie, 2000).\smallskip


\noindent{\bf PTL \textit{vs}. random selection.} In the previous analysis, two conflicting observations were found regarding the comparison between PTL and random selection. Firstly, PTL consistently provides better accuracy than random selection, regardless of training settings, for both the same domain and cross-domain tasks (Fig.~\ref{fig:scaling_behavior_of_synthimg}). On the other hand, random selection is generally more effective in reducing the distribution gap using synthetic data than PTL (Tab.~\ref{tab:distribution_gap_with_various_synthetic_images}). When selecting synthetic images from the synthetic pool, PTL focuses more on synthetic images with similar characteristics to the reference dataset more frequently than simply increasing the generalization ability of the training set. As this selection strategy is proposed to prevent degradation of the sim2real transformation quality, using higher-quality transformed synthetic images in training has a positive impact on increasing detection accuracy.

\input{Tables/distribution_gap_various_synthetic_images}



\subsection{A Study on the Impact of the Synthetic Data Pool} 

For the third study, we explored the inherent properties of the synthetic data pool that in turn influence the use of synthetic data.\smallskip

\noindent{\bf Accuracy comparison \wrt rendering parameters.} Our synthetic data pool, the Archangel-Synthetic dataset, was built to show various human appearances captured with a virtual UAV by controlling several rendering parameters in a simulation space (altitudes and radii of camera location, camera viewing angles, and human characters and poses). To examine the effect of each parameter on using synthetic data, we construct five subsets of the synthetic data pool, where each is built more sparsely for one parameter while fixing the values of other parameters. Each sub-pool includes the synthetic data with sparsely and regularly sampled altitudes (SAlt), radii (SRad), viewing angles (SAng), human characters (SCha), or human poses (SPos). In addition to the regularly sampled sub-pools, we also construct extremely biased sampled sub-pools along the three parameters: altitudes, radii, and viewing angles. For altitude and radii, subsets (BSAlt and BSRad) were constructed by collecting images assuming that the camera location is far away, and for viewing angle, a subset (BSAng) was constructed with only images with the front view of a person. These additional sub-pools can be used to investigate the impact of low-diversity synthetic pools when leveraging synthetic data in training.\footnote{Details on how to build subsets of the synthetic data pool are provided in the supplementary material.}

In Table~\ref{tab:comparison_synthetic_pool}, we compare the detection accuracy of the original pool and its five subsets. `SPos' exhibits significantly lower accuracy than the original, while the other four subsets show similar or even higher accuracy. In sampling the synthetic pool, reducing the variety of human poses significantly decreases detection accuracy as it leads to the inability to cover a wide range of human poses in test data. However, the decrease in accuracy is not observed when using subsets of synthetic data linked to the sparse sampling of other parameters.\smallskip

\noindent{\bf Properties of the synthetic pool.} We introduce several metrics to understand the variation in the ability of the synthetic pool to cover a variety of human appearances, depending on the rendering parameters, when used sparsely. We firstly consider \emph{how densely data is located in the feature space} (density) and \emph{how diverse the data distribution is in the feature space} (diversity). Specifically, the density and diversity of the pool $\mathcal{P}$ can be defined as below:

\begin{itemize}
\item density:
\begin{equation}
\frac{1}{|\text{adj}(\mathcal{P})|}\!\!\!\!\!\!\!\!\!\sum_{~~~~~~{\bf p},{\bf q}\in\text{adj}(\mathcal{P})}{\!\!\!\!\!\!f({\bf p})^\top f({\bf q})}.
\label{eq:density}
\end{equation}

\item diversity:
\begin{equation}
\frac{1}{|\mathcal{P}|}\sum_{{\bf x}\in\mathcal{P}}{||f({\bf x})-\mu||_2^k}.
\label{eq:diversity}
\end{equation}
\end{itemize}

\noindent $f(\cdot)$ is the embedding in the feature space of the detector. Here, we use a detector trained without the synthetic data to avoid the influence of them used in training when measuring the properties of the pool. $\text{adj}(\mathcal{P})$ includes all data pairs associated with different neighboring values from each rendering parameter while others are fixed. Intuitively, a high $f({\bf p})^\top f({\bf q})$ in eq.~\ref{eq:density} indicates that ${\bf p}$ and ${\bf q}$ lie close to each other in the feature space. $\mu$ is the mean feature over all data points in $\mathcal{P}$ (\ie, $\mu=\sum_{{\bf x}\in \mathcal{P}}{f({\bf x})}$). $k$ is a hyper-parameter that controls how each data point deviates from $\mu$ when calculating diversity. Higher $k$ leads to more weights on the data points away from $\mu$. (We use $k=10$). We also consider the domain gap between the synthetic pool and the reference dataset, which can be calculated in a similar way to measuring the distribution gap (eq.~\ref{eq:distribution gap}).

In Table~\ref{tab:comparison_synthetic_pool}, three sub-pools (`SPos', `BSAlt', and `BSRad'), which showed significantly lower accuracy than the original pool, have the following properties: higher density, less diversity, and closer domain gap to the reference dataset than the original and other pools. This strongly indicates that \emph{sampling synthetic data from a denser but less diverse distribution adversely affects using synthetic data in training, leading to low accuracy}. Moreover, `BSAlt', which presents very low accuracy, has a very large domain gap to the reference data. Using synthetic pools with large domain gaps to the reference data adversely impacts accuracy in both same-domain and cross-domain tasks. Unexpectedly, when `BSAng' was used, detection accuracy did not decrease, and the properties of the synthetic pool were normal. This is probably because the reference (real) data and other test real datasets also contain images of people looking straight ahead.


\smallskip

\noindent{\bf Analysis in terms of distribution gaps.} In Table~\ref{tab:comparison_synthetic_pool}, using `SPos', `BSAlt', or `BSAng' results in a larger distribution gap for cross-domain datasets than using other pools. This is aligned well with our previous analyses.

\input{Tables/comparison_synthetic_pool}

==> Styles/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Tables/distribution_gap.tex <==
%\begin{table}[t]
\caption{{\bf Distribution gaps of various datasets} from VisDrone. The better accuracy between using and not using synthetic images is shown in bold.}
\label{tab:distribution_gap}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{9.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rr|rr|rr|rr}
& & \multicolumn{2}{c|}{Okutama} & \multicolumn{2}{c|}{ICG} & \multicolumn{2}{c|}{HERIDAL} & \multicolumn{2}{c}{SARD} \\
setup & w/ synth & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c|}{all} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c|}{all} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c|}{all} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c}{all} \\\hline
\multirow{2}{*}{Vis-20} & & 90.6 & 4,627.1 & 63.0 & 2,372.9 & 151.0 & 6,524.2 & 132.2 & 5,083.5 \\
& \textcolor{red}{\checkmark} & {\bf 35.1} & {\bf 487.9} & {\bf 39.4} & {\bf 518.2} & {\bf 40.8} & {\bf 406.9} & {\bf 36.8} & {\bf 420.3} \\\hline
\multirow{2}{*}{Vis-50} & & 40.3 & {\bf 274.0} & 32.8 & {\bf 285.6} & 62.7 & {\bf 340.5} & 40.7 & {\bf 323.0} \\
& \textcolor{red}{\checkmark} & {\bf 31.7} & 431.1 & {\bf 31.9} & 368.7 & {\bf 35.3} & 639.1 & {\bf 33.6} & 958.4 \\\hline
\multirow{2}{*}{Vis-100} & & 36.3 & 119.4 & 32.3 & {\bf 103.1} & 58.5 & 190.0 & 63.2 & {\bf 222.0} \\
& \textcolor{red}{\checkmark} & {\bf 23.2} & {\bf 82.7} & {\bf 28.0} & 182.4 & {\bf 27.7} & {\bf 177.9} & {\bf 27.6} & 300.7 \\\hline
\multirow{2}{*}{Vis-200} & & 27.4 & 167.1 & 29.3 & {\bf 103.5} & 40.6 & {\bf 130.2} & 38.8 & {\bf 122.8} \\
& \textcolor{red}{\checkmark} & {\bf 19.8} & {\bf 159.5} & {\bf 22.5} & 207.7 & {\bf 27.2} & 305.4 & {\bf 25.8} & 424.5 \\
\end{tabular}
}
%\end{table}

==> Tables/scalability_realimg_detail_twocolumn.tex <==
\begin{table*}[t]
\caption{{\bf Numerical results with the size of real dataset}. In each bin presenting accuracy, the mean and standard deviation of AP@.5 and AP@[.5:.95] calculated over 3 runs are reported.}
\label{tab:scalability_realimg}
\begin{subtable}[b]{\linewidth}
\captionsetup{type=table}
\caption{Same-domain and cross-domain accuracy in the Vis-$N$}
\label{tab:accuracy_scalability_of_realimg}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{6.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rrrrr}
\multicolumn{1}{c|}{setup} & w/ synth & \multicolumn{1}{c}{VisDrone} & \multicolumn{1}{c}{Okutama} & \multicolumn{1}{c}{ICG} & \multicolumn{1}{c}{HERIDAL} & \multicolumn{1}{c}{SARD} \\\hline
\multirow{2}{*}{Vis-20} & & 3.43\textcolor{gray}{{\scriptsize $\pm$0.57}} / 0.98\textcolor{gray}{{\scriptsize $\pm$0.12}} & 18.38\textcolor{gray}{{\scriptsize $\pm$8.74}} / ~~4.73\textcolor{gray}{{\scriptsize $\pm$2.61}} & 2.14\textcolor{gray}{{\scriptsize $\pm$0.70}} / ~~0.43\textcolor{gray}{{\scriptsize $\pm$0.15}} & 7.11\textcolor{gray}{{\scriptsize $\pm$3.45}} / ~~2.13\textcolor{gray}{{\scriptsize $\pm$1.08}} & 7.24\textcolor{gray}{{\scriptsize $\pm$3.32}} / ~~2.07\textcolor{gray}{{\scriptsize $\pm$1.14}} \\
& \textcolor{red}{\checkmark} & 6.18\textcolor{gray}{{\scriptsize $\pm$0.47}} / 1.82\textcolor{gray}{{\scriptsize $\pm$0.33}} & 29.93\textcolor{gray}{{\scriptsize $\pm$3.01}} / ~~7.18\textcolor{gray}{{\scriptsize $\pm$0.90}} & 29.30\textcolor{gray}{{\scriptsize $\pm$2.70}} / ~~8.09\textcolor{gray}{{\scriptsize $\pm$0.33}} & 28.61\textcolor{gray}{{\scriptsize $\pm$2.91}} / ~~9.57\textcolor{gray}{{\scriptsize $\pm$1.13}} & 34.96\textcolor{gray}{{\scriptsize $\pm$3.26}} / 11.53\textcolor{gray}{{\scriptsize $\pm$1.06}}\\\hline
\multirow{2}{*}{Vis-50} & & 6.13\textcolor{gray}{{\scriptsize $\pm$0.28}} / 1.84\textcolor{gray}{{\scriptsize $\pm$0.21}} & 25.65\textcolor{gray}{{\scriptsize $\pm$4.62}} / ~~6.98\textcolor{gray}{{\scriptsize $\pm$1.56}} & 6.57\textcolor{gray}{{\scriptsize $\pm$2.41}} / ~~1.48\textcolor{gray}{{\scriptsize $\pm$0.89}} & 12.12\textcolor{gray}{{\scriptsize $\pm$3.35}} / ~~3.93\textcolor{gray}{{\scriptsize $\pm$1.17}} & 17.73\textcolor{gray}{{\scriptsize $\pm$1.58}} / ~~4.92\textcolor{gray}{{\scriptsize $\pm$0.61}} \\
& \textcolor{red}{\checkmark} & 8.91\textcolor{gray}{{\scriptsize $\pm$0.20}} / 2.79\textcolor{gray}{{\scriptsize $\pm$0.08}} & 37.67\textcolor{gray}{{\scriptsize $\pm$0.59}} / ~~9.80\textcolor{gray}{{\scriptsize $\pm$0.25}} & 32.86\textcolor{gray}{{\scriptsize $\pm$5.36}} / ~~9.64\textcolor{gray}{{\scriptsize $\pm$2.03}} & 36.88\textcolor{gray}{{\scriptsize $\pm$3.79}} / 12.16\textcolor{gray}{{\scriptsize $\pm$1.93}} & 45.75\textcolor{gray}{{\scriptsize $\pm$2.16}} / 15.92\textcolor{gray}{{\scriptsize $\pm$1.73}}\\\hline
\multirow{2}{*}{Vis-100} & & 7.91\textcolor{gray}{{\scriptsize $\pm$0.13}} / 2.36\textcolor{gray}{{\scriptsize $\pm$0.07}} & 31.37\textcolor{gray}{{\scriptsize $\pm$1.49}} / ~~8.21\textcolor{gray}{{\scriptsize $\pm$0.29}} & 7.60\textcolor{gray}{{\scriptsize $\pm$1.51}} / ~~1.81\textcolor{gray}{{\scriptsize $\pm$0.32}} & 14.64\textcolor{gray}{{\scriptsize $\pm$6.04}} / ~~4.59\textcolor{gray}{{\scriptsize $\pm$1.47}} & 18.27\textcolor{gray}{{\scriptsize $\pm$1.25}} / ~~5.42\textcolor{gray}{{\scriptsize $\pm$0.50}} \\
& \textcolor{red}{\checkmark} & 10.56\textcolor{gray}{{\scriptsize $\pm$0.49}} / 3.29\textcolor{gray}{{\scriptsize $\pm$0.23}} & 41.18\textcolor{gray}{{\scriptsize $\pm$3.35}} / 10.86\textcolor{gray}{{\scriptsize $\pm$1.07}} & 35.69\textcolor{gray}{{\scriptsize $\pm$1.65}} / 11.02\textcolor{gray}{{\scriptsize $\pm$1.35}} & 38.54\textcolor{gray}{{\scriptsize $\pm$7.75}} / 13.37\textcolor{gray}{{\scriptsize $\pm$2.36}} & 48.15\textcolor{gray}{{\scriptsize $\pm$1.18}} / 17.05\textcolor{gray}{{\scriptsize $\pm$0.87}}\\\hline
\multirow{2}{*}{Vis-200} & & 10.55\textcolor{gray}{{\scriptsize $\pm$1.41}} / 3.18\textcolor{gray}{{\scriptsize $\pm$0.55}} & 38.58\textcolor{gray}{{\scriptsize $\pm$4.81}} / 10.25\textcolor{gray}{{\scriptsize $\pm$1.66}} & 6.50\textcolor{gray}{{\scriptsize $\pm$3.17}} / ~~1.39\textcolor{gray}{{\scriptsize $\pm$0.63}} & 14.76\textcolor{gray}{{\scriptsize $\pm$9.76}} / ~~4.68\textcolor{gray}{{\scriptsize $\pm$2.72}} & 21.87\textcolor{gray}{{\scriptsize $\pm$7.48}} / ~~6.98\textcolor{gray}{{\scriptsize $\pm$1.97}} \\
& \textcolor{red}{\checkmark} & 12.78\textcolor{gray}{{\scriptsize $\pm$0.48}} / 4.10\textcolor{gray}{{\scriptsize $\pm$0.28}} & 46.62\textcolor{gray}{{\scriptsize $\pm$0.93}} / 12.37\textcolor{gray}{{\scriptsize $\pm$0.21}} & 30.48\textcolor{gray}{{\scriptsize $\pm$0.34}} / ~~8.21\textcolor{gray}{{\scriptsize $\pm$0.43}} & 37.60\textcolor{gray}{{\scriptsize $\pm$2.12}} / 13.74\textcolor{gray}{{\scriptsize $\pm$1.46}} & 49.60\textcolor{gray}{{\scriptsize $\pm$1.78}} / 17.73\textcolor{gray}{{\scriptsize $\pm$0.49}}\\
\end{tabular}
}
\end{subtable}
\\\\\\
\begin{subtable}[b]{\linewidth}
\captionsetup{type=table}
\caption{Same-domain accuracy w/o synthetic data and its ratio to the Vis-$N$ (w/ synthetic data) when using the same number of real images}
\label{tab:ratio_scalability_of_realimg}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{8.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rrrr}
& & \multicolumn{4}{c}{\# of real image} \\
& testset & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{50} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{200} \\\hline
accuracy & \multirow{2}{*}{Okutama} & 37.93\textcolor{gray}{{\scriptsize $\pm$1.75}} / ~~9.93\textcolor{gray}{{\scriptsize $\pm$0.16}} & 51.31\textcolor{gray}{{\scriptsize $\pm$2.05}} / 14.13\textcolor{gray}{{\scriptsize $\pm$0.90}} & 55.98\textcolor{gray}{{\scriptsize $\pm$0.75}} / 16.68\textcolor{gray}{{\scriptsize $\pm$0.45}} & 64.76\textcolor{gray}{{\scriptsize $\pm$0.97}} / 20.28\textcolor{gray}{{\scriptsize $\pm$0.17}}\\
ratio to Vis-$N$ (w/ synth) & & \multicolumn{1}{c}{0.79 / 0.72} & \multicolumn{1}{c}{0.73 / 0.69} & \multicolumn{1}{c}{0.74 / 0.65} & \multicolumn{1}{c}{0.72 / 0.61} \\\hline
accuracy & \multirow{2}{*}{ICG} & 40.36\textcolor{gray}{{\scriptsize $\pm$0.96}} / 10.63\textcolor{gray}{{\scriptsize $\pm$0.38}} & 60.95\textcolor{gray}{{\scriptsize $\pm$1.76}} / 19.57\textcolor{gray}{{\scriptsize $\pm$1.19}} & 73.23\textcolor{gray}{{\scriptsize $\pm$0.76}} / 27.53\textcolor{gray}{{\scriptsize $\pm$0.95}} & 84.21\textcolor{gray}{{\scriptsize $\pm$1.50}} / 35.98\textcolor{gray}{{\scriptsize $\pm$1.20}}\\
ratio to Vis-$N$ (w/ synth) & & \multicolumn{1}{c}{0.73 / 0.76} & \multicolumn{1}{c}{0.54 / 0.49} & \multicolumn{1}{c}{0.49 / 0.40} & \multicolumn{1}{c}{0.36 / 0.23} \\\hline
accuracy & \multirow{2}{*}{HERIDAL} & 41.39\textcolor{gray}{{\scriptsize $\pm$2.86}} / 12.75\textcolor{gray}{{\scriptsize $\pm$1.82}} & 58.97\textcolor{gray}{{\scriptsize $\pm$2.86}} / 19.76\textcolor{gray}{{\scriptsize $\pm$0.96}} & 65.78\textcolor{gray}{{\scriptsize $\pm$0.70}} / 26.27\textcolor{gray}{{\scriptsize $\pm$1.25}} & 71.53\textcolor{gray}{{\scriptsize $\pm$0.49}} / 31.18\textcolor{gray}{{\scriptsize $\pm$1.70}}\\
ratio to Vis-$N$ (w/ synth) & & \multicolumn{1}{c}{0.69 / 0.75} & \multicolumn{1}{c}{0.63 / 0.62} & \multicolumn{1}{c}{0.59 / 0.51} & \multicolumn{1}{c}{0.53 / 0.44} \\\hline
accuracy & \multirow{2}{*}{SARD} & 33.44\textcolor{gray}{{\scriptsize $\pm$6.36}} / ~~8.52\textcolor{gray}{{\scriptsize $\pm$2.20}} & 51.35\textcolor{gray}{{\scriptsize $\pm$1.68}} / 15.28\textcolor{gray}{{\scriptsize $\pm$0.78}} & 66.81\textcolor{gray}{{\scriptsize $\pm$3.15}} / 23.75\textcolor{gray}{{\scriptsize $\pm$1.79}} & 75.76\textcolor{gray}{{\scriptsize $\pm$1.62}} / 30.17\textcolor{gray}{{\scriptsize $\pm$0.98}}\\
ratio to Vis-$N$ (w/ synth) & & \multicolumn{1}{c}{1.05 / 1.35} & \multicolumn{1}{c}{0.89 / 1.04} & \multicolumn{1}{c}{0.72 / 0.72} & \multicolumn{1}{c}{0.65 / 0.59} \\
\end{tabular}
}
\end{subtable}

\end{table*}

==> Tables/scalability_synthimg_detail_twocolumn.tex <==
\begin{table*}[t]
\caption{{\bf Numerical results with the size of synthetic dataset.} `Random' denotes random selection.}
\label{tab:scalability_synthimg}
\begin{subtable}[b]{\linewidth}
\captionsetup{type=table}
\caption{Vis-20}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rrrrr}
& & \multicolumn{5}{c}{\# of synthetic image} \\
\multicolumn{1}{c|}{method} & test set & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{2000} \\\hline
PTL & \multirow{2}{*}{VisDrone} & \multirow{2}{*}{3.43\textcolor{gray}{{\scriptsize $\pm$0.57}} /~~0.98\textcolor{gray}{{\scriptsize $\pm$0.12}}} & 5.88\textcolor{gray}{{\scriptsize $\pm$0.58}} /~~1.73\textcolor{gray}{{\scriptsize $\pm$0.21}} & 6.48\textcolor{gray}{{\scriptsize $\pm$0.56}} /~~1.89\textcolor{gray}{{\scriptsize $\pm$0.13}} & 6.28\textcolor{gray}{{\scriptsize $\pm$0.86}} /~~1.76\textcolor{gray}{{\scriptsize $\pm$0.28}} & 6.18\textcolor{gray}{{\scriptsize $\pm$0.47}} /~~1.82\textcolor{gray}{{\scriptsize $\pm$0.33}} \\
Random & & & 5.90\textcolor{gray}{{\scriptsize $\pm$0.29}} /~~1.63\textcolor{gray}{{\scriptsize $\pm$0.07}} & 6.40\textcolor{gray}{{\scriptsize $\pm$0.85}} /~~1.79\textcolor{gray}{{\scriptsize $\pm$0.28}} & 6.41\textcolor{gray}{{\scriptsize $\pm$0.20}} /~~1.85\textcolor{gray}{{\scriptsize $\pm$0.09}} & 6.09\textcolor{gray}{{\scriptsize $\pm$0.69}} /~~1.75\textcolor{gray}{{\scriptsize $\pm$0.28}} \\\hline
PTL & \multirow{2}{*}{Okutama} & \multirow{2}{*}{18.38\textcolor{gray}{{\scriptsize $\pm$8.74}} /~~4.73\textcolor{gray}{{\scriptsize $\pm$2.61}}} & 28.01\textcolor{gray}{{\scriptsize $\pm$2.89}} /~~6.73\textcolor{gray}{{\scriptsize $\pm$0.80}} & 30.54\textcolor{gray}{{\scriptsize $\pm$1.06}} /~~7.24\textcolor{gray}{{\scriptsize $\pm$0.36}} & 29.63\textcolor{gray}{{\scriptsize $\pm$1.21}} /~~6.90\textcolor{gray}{{\scriptsize $\pm$0.41}} & 29.93\textcolor{gray}{{\scriptsize $\pm$3.01}} /~~7.18\textcolor{gray}{{\scriptsize $\pm$0.90}} \\
Random & & & 27.54\textcolor{gray}{{\scriptsize $\pm$1.40}} /~~6.18\textcolor{gray}{{\scriptsize $\pm$0.62}} & 28.20\textcolor{gray}{{\scriptsize $\pm$1.74}} /~~6.30\textcolor{gray}{{\scriptsize $\pm$0.34}} & 27.20\textcolor{gray}{{\scriptsize $\pm$0.90}} /~~6.08\textcolor{gray}{{\scriptsize $\pm$0.24}} & 27.80\textcolor{gray}{{\scriptsize $\pm$3.03}} /~~6.08\textcolor{gray}{{\scriptsize $\pm$0.99}} \\\hline
PTL & \multirow{2}{*}{ICG} & \multirow{2}{*}{2.14\textcolor{gray}{{\scriptsize $\pm$0.70}} /~~0.43\textcolor{gray}{{\scriptsize $\pm$0.15}}} & 15.16\textcolor{gray}{{\scriptsize $\pm$3.85}} /~~3.58\textcolor{gray}{{\scriptsize $\pm$1.24}} & 23.03\textcolor{gray}{{\scriptsize $\pm$4.68}} /~~6.13\textcolor{gray}{{\scriptsize $\pm$1.79}} & 26.70\textcolor{gray}{{\scriptsize $\pm$1.86}} /~~7.47\textcolor{gray}{{\scriptsize $\pm$1.37}} & 29.30\textcolor{gray}{{\scriptsize $\pm$2.70}} /~~8.09\textcolor{gray}{{\scriptsize $\pm$0.33}} \\
Random & & & 8.97\textcolor{gray}{{\scriptsize $\pm$0.67}} /~~1.97\textcolor{gray}{{\scriptsize $\pm$0.20}} & 29.62\textcolor{gray}{{\scriptsize $\pm$2.03}} /~~8.06\textcolor{gray}{{\scriptsize $\pm$0.30}} & 26.69\textcolor{gray}{{\scriptsize $\pm$6.21}} /~~7.39\textcolor{gray}{{\scriptsize $\pm$1.14}} & 33.70\textcolor{gray}{{\scriptsize $\pm$0.85}} /~~9.54\textcolor{gray}{{\scriptsize $\pm$0.87}} \\\hline
PTL & \multirow{2}{*}{HERIDAL} & \multirow{2}{*}{7.11\textcolor{gray}{{\scriptsize $\pm$3.45}} /~~2.13\textcolor{gray}{{\scriptsize $\pm$1.08}}} & 20.24\textcolor{gray}{{\scriptsize $\pm$3.85}} /~~5.87\textcolor{gray}{{\scriptsize $\pm$1.83}} & 26.50\textcolor{gray}{{\scriptsize $\pm$3.02}} /~~7.86\textcolor{gray}{{\scriptsize $\pm$1.10}} & 26.98\textcolor{gray}{{\scriptsize $\pm$5.38}} /~~8.49\textcolor{gray}{{\scriptsize $\pm$1.14}} & 28.61\textcolor{gray}{{\scriptsize $\pm$2.91}} /~~9.57\textcolor{gray}{{\scriptsize $\pm$1.13}} \\
Random & & & 14.82\textcolor{gray}{{\scriptsize $\pm$2.57}} /~~3.94\textcolor{gray}{{\scriptsize $\pm$1.00}} & 23.37\textcolor{gray}{{\scriptsize $\pm$2.19}} /~~6.77\textcolor{gray}{{\scriptsize $\pm$0.92}} & 25.98\textcolor{gray}{{\scriptsize $\pm$2.92}} /~~7.41\textcolor{gray}{{\scriptsize $\pm$0.73}} & 29.22\textcolor{gray}{{\scriptsize $\pm$4.55}} /~~9.02\textcolor{gray}{{\scriptsize $\pm$1.95}} \\\hline
PTL & \multirow{2}{*}{SARD} & \multirow{2}{*}{7.24\textcolor{gray}{{\scriptsize $\pm$3.32}} /~~2.07\textcolor{gray}{{\scriptsize $\pm$1.14}}} & 24.51\textcolor{gray}{{\scriptsize $\pm$3.39}} /~~7.37\textcolor{gray}{{\scriptsize $\pm$1.33}} & 34.74\textcolor{gray}{{\scriptsize $\pm$1.93}} /11.11\textcolor{gray}{{\scriptsize $\pm$1.14}} & 35.65\textcolor{gray}{{\scriptsize $\pm$3.07}} /11.90\textcolor{gray}{{\scriptsize $\pm$0.78}} & 34.96\textcolor{gray}{{\scriptsize $\pm$3.26}} /11.53\textcolor{gray}{{\scriptsize $\pm$1.06}} \\
Random & & & 22.15\textcolor{gray}{{\scriptsize $\pm$3.13}} /~~6.52\textcolor{gray}{{\scriptsize $\pm$1.44}} & 34.98\textcolor{gray}{{\scriptsize $\pm$5.04}} /11.18\textcolor{gray}{{\scriptsize $\pm$1.77}} & 37.35\textcolor{gray}{{\scriptsize $\pm$3.35}} /11.78\textcolor{gray}{{\scriptsize $\pm$0.67}} & 40.01\textcolor{gray}{{\scriptsize $\pm$2.07}} /13.36\textcolor{gray}{{\scriptsize $\pm$0.85}} \\
\end{tabular}
}
\end{subtable}
\\\\\\
\begin{subtable}[b]{\linewidth}
\captionsetup{type=table}
\caption{Vis-50}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rrrrr}
& & \multicolumn{5}{c}{\# of synthetic image} \\
\multicolumn{1}{c|}{method} & test set & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{2000} \\\hline
PTL & \multirow{2}{*}{VisDrone} & \multirow{2}{*}{6.13\textcolor{gray}{{\scriptsize $\pm$0.28}} /~~1.84\textcolor{gray}{{\scriptsize $\pm$0.21}}} & 8.48\textcolor{gray}{{\scriptsize $\pm$0.26}} /~~2.55\textcolor{gray}{{\scriptsize $\pm$0.10}} & 9.27\textcolor{gray}{{\scriptsize $\pm$0.29}} /~~2.84\textcolor{gray}{{\scriptsize $\pm$0.12}} & 9.39\textcolor{gray}{{\scriptsize $\pm$0.12}} /~~2.98\textcolor{gray}{{\scriptsize $\pm$0.07}} & 8.91\textcolor{gray}{{\scriptsize $\pm$0.20}} /~~2.79\textcolor{gray}{{\scriptsize $\pm$0.08}} \\
Random & & & 8.17\textcolor{gray}{{\scriptsize $\pm$0.28}} /~~2.43\textcolor{gray}{{\scriptsize $\pm$0.22}} & 9.23\textcolor{gray}{{\scriptsize $\pm$0.29}} /~~2.77\textcolor{gray}{{\scriptsize $\pm$0.15}} & 8.97\textcolor{gray}{{\scriptsize $\pm$0.08}} /~~2.70\textcolor{gray}{{\scriptsize $\pm$0.11}} & 9.01\textcolor{gray}{{\scriptsize $\pm$0.56}} /~~2.69\textcolor{gray}{{\scriptsize $\pm$0.04}} \\\hline
PTL & \multirow{2}{*}{Okutama} & \multirow{2}{*}{25.65\textcolor{gray}{{\scriptsize $\pm$4.62}} /~~6.98\textcolor{gray}{{\scriptsize $\pm$1.56}}} & 35.21\textcolor{gray}{{\scriptsize $\pm$4.67}} /~~9.45\textcolor{gray}{{\scriptsize $\pm$1.70}} & 37.94\textcolor{gray}{{\scriptsize $\pm$1.84}} /~~9.88\textcolor{gray}{{\scriptsize $\pm$0.76}} & 37.17\textcolor{gray}{{\scriptsize $\pm$2.10}} /~~9.63\textcolor{gray}{{\scriptsize $\pm$0.95}} & 38.85\textcolor{gray}{{\scriptsize $\pm$3.34}} /10.04\textcolor{gray}{{\scriptsize $\pm$1.10}} \\
Random & & & 32.66\textcolor{gray}{{\scriptsize $\pm$5.86}} /~~8.46\textcolor{gray}{{\scriptsize $\pm$1.92}} & 34.48\textcolor{gray}{{\scriptsize $\pm$5.68}} /~~8.44\textcolor{gray}{{\scriptsize $\pm$2.03}} & 33.68\textcolor{gray}{{\scriptsize $\pm$6.44}} /~~8.12\textcolor{gray}{{\scriptsize $\pm$2.04}} & 33.29\textcolor{gray}{{\scriptsize $\pm$4.53}} /~~7.92\textcolor{gray}{{\scriptsize $\pm$1.20}} \\\hline
PTL & \multirow{2}{*}{ICG} & \multirow{2}{*}{6.57\textcolor{gray}{{\scriptsize $\pm$2.41}} /~~1.48\textcolor{gray}{{\scriptsize $\pm$0.89}}}& 16.87\textcolor{gray}{{\scriptsize $\pm$2.23}} /~~4.16\textcolor{gray}{{\scriptsize $\pm$0.71}} & 29.70\textcolor{gray}{{\scriptsize $\pm$3.13}} /~~7.27\textcolor{gray}{{\scriptsize $\pm$1.27}} & 30.94\textcolor{gray}{{\scriptsize $\pm$6.70}} /~~8.57\textcolor{gray}{{\scriptsize $\pm$2.54}} & 32.86\textcolor{gray}{{\scriptsize $\pm$5.36}} /~~9.64\textcolor{gray}{{\scriptsize $\pm$2.03}} \\
Random & & & 14.43\textcolor{gray}{{\scriptsize $\pm$2.72}} /~~3.24\textcolor{gray}{{\scriptsize $\pm$0.90}} & 28.78\textcolor{gray}{{\scriptsize $\pm$4.90}} /~~7.05\textcolor{gray}{{\scriptsize $\pm$1.65}} & 31.45\textcolor{gray}{{\scriptsize $\pm$1.49}} /~~8.72\textcolor{gray}{{\scriptsize $\pm$1.44}} & 35.51\textcolor{gray}{{\scriptsize $\pm$2.12}} /~~9.69\textcolor{gray}{{\scriptsize $\pm$0.33}} \\\hline
PTL & \multirow{2}{*}{HERIDAL} & \multirow{2}{*}{12.12\textcolor{gray}{{\scriptsize $\pm$3.35}} /~~3.93\textcolor{gray}{{\scriptsize $\pm$1.17}}} & 22.81\textcolor{gray}{{\scriptsize $\pm$1.43}} /~~7.22\textcolor{gray}{{\scriptsize $\pm$0.59}} & 31.62\textcolor{gray}{{\scriptsize $\pm$1.32}} /10.27\textcolor{gray}{{\scriptsize $\pm$0.74}} & 33.24\textcolor{gray}{{\scriptsize $\pm$1.66}} /11.31\textcolor{gray}{{\scriptsize $\pm$1.30}} & 36.88\textcolor{gray}{{\scriptsize $\pm$3.79}} /12.16\textcolor{gray}{{\scriptsize $\pm$1.93}} \\
Random & & & 21.71\textcolor{gray}{{\scriptsize $\pm$2.14}} /~~6.56\textcolor{gray}{{\scriptsize $\pm$0.72}} & 29.87\textcolor{gray}{{\scriptsize $\pm$3.93}} /~~9.73\textcolor{gray}{{\scriptsize $\pm$1.39}} & 32.11\textcolor{gray}{{\scriptsize $\pm$5.48}} /10.41\textcolor{gray}{{\scriptsize $\pm$2.96}} & 34.06\textcolor{gray}{{\scriptsize $\pm$5.59}} /11.08\textcolor{gray}{{\scriptsize $\pm$2.31}} \\\hline
PTL & \multirow{2}{*}{SARD} & \multirow{2}{*}{17.73\textcolor{gray}{{\scriptsize $\pm$1.58}} /~~4.92\textcolor{gray}{{\scriptsize $\pm$0.61}}} & 32.18\textcolor{gray}{{\scriptsize $\pm$3.75}} /~~9.77\textcolor{gray}{{\scriptsize $\pm$1.06}} & 43.67\textcolor{gray}{{\scriptsize $\pm$4.01}} /14.33\textcolor{gray}{{\scriptsize $\pm$1.66}} & 43.59\textcolor{gray}{{\scriptsize $\pm$2.31}} /14.15\textcolor{gray}{{\scriptsize $\pm$2.17}} & 45.75\textcolor{gray}{{\scriptsize $\pm$2.16}} /15.92\textcolor{gray}{{\scriptsize $\pm$1.73}} \\
Random & & & 30.74\textcolor{gray}{{\scriptsize $\pm$1.61}} /~~9.41\textcolor{gray}{{\scriptsize $\pm$0.65}} & 38.52\textcolor{gray}{{\scriptsize $\pm$0.88}} /12.10\textcolor{gray}{{\scriptsize $\pm$0.96}} & 44.28\textcolor{gray}{{\scriptsize $\pm$2.83}} /14.30\textcolor{gray}{{\scriptsize $\pm$1.68}} & 45.56\textcolor{gray}{{\scriptsize $\pm$3.26}} /15.21\textcolor{gray}{{\scriptsize $\pm$1.64}} \\
\end{tabular}
}
\end{subtable}
\\\\\\
\begin{subtable}[b]{\linewidth}
\captionsetup{type=table}
\caption{Vis-100}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rrrrr}
& & \multicolumn{5}{c}{\# of synthetic image} \\
\multicolumn{1}{c|}{method} & test set & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{2000} \\\hline
PTL & \multirow{2}{*}{VisDrone} & \multirow{2}{*}{7.91\textcolor{gray}{{\scriptsize $\pm$0.13}} /~~2.36\textcolor{gray}{{\scriptsize $\pm$0.07}}} & 9.58\textcolor{gray}{{\scriptsize $\pm$0.57}} /~~2.94\textcolor{gray}{{\scriptsize $\pm$0.21}} & 10.79\textcolor{gray}{{\scriptsize $\pm$0.28}} /~~3.40\textcolor{gray}{{\scriptsize $\pm$0.09}} & 10.82\textcolor{gray}{{\scriptsize $\pm$0.45}} /~~3.41\textcolor{gray}{{\scriptsize $\pm$0.07}} & 10.56\textcolor{gray}{{\scriptsize $\pm$0.49}} /~~3.29\textcolor{gray}{{\scriptsize $\pm$0.23}} \\
Random & & & 9.13\textcolor{gray}{{\scriptsize $\pm$0.60}} /~~2.64\textcolor{gray}{{\scriptsize $\pm$0.16}} & 10.66\textcolor{gray}{{\scriptsize $\pm$0.10}} /~~3.23\textcolor{gray}{{\scriptsize $\pm$0.09}} & 10.67\textcolor{gray}{{\scriptsize $\pm$0.43}} /~~3.28\textcolor{gray}{{\scriptsize $\pm$0.14}} & 10.13\textcolor{gray}{{\scriptsize $\pm$0.27}} /~~3.11\textcolor{gray}{{\scriptsize $\pm$0.03}} \\\hline
PTL & \multirow{2}{*}{Okutama} & \multirow{2}{*}{31.37\textcolor{gray}{{\scriptsize $\pm$1.49}} /~~8.21\textcolor{gray}{{\scriptsize $\pm$0.29}}} & 36.61\textcolor{gray}{{\scriptsize $\pm$4.46}} /~~9.89\textcolor{gray}{{\scriptsize $\pm$1.28}} & 40.37\textcolor{gray}{{\scriptsize $\pm$4.12}} /10.41\textcolor{gray}{{\scriptsize $\pm$0.91}} & 40.76\textcolor{gray}{{\scriptsize $\pm$4.69}} /10.48\textcolor{gray}{{\scriptsize $\pm$1.12}} & 41.18\textcolor{gray}{{\scriptsize $\pm$3.35}} /10.86\textcolor{gray}{{\scriptsize $\pm$1.07}} \\
Random & & & 34.92\textcolor{gray}{{\scriptsize $\pm$2.86}} /~~9.05\textcolor{gray}{{\scriptsize $\pm$0.85}} & 38.12\textcolor{gray}{{\scriptsize $\pm$2.66}} /~~9.51\textcolor{gray}{{\scriptsize $\pm$0.42}} & 38.80\textcolor{gray}{{\scriptsize $\pm$2.42}} /~~9.77\textcolor{gray}{{\scriptsize $\pm$0.26}} & 38.18\textcolor{gray}{{\scriptsize $\pm$1.79}} /~~9.50\textcolor{gray}{{\scriptsize $\pm$0.40}} \\\hline
PTL & \multirow{2}{*}{ICG} & \multirow{2}{*}{7.60\textcolor{gray}{{\scriptsize $\pm$1.51}} /~~1.81\textcolor{gray}{{\scriptsize $\pm$0.32}}} & 18.19\textcolor{gray}{{\scriptsize $\pm$3.47}} /~~4.47\textcolor{gray}{{\scriptsize $\pm$0.92}} & 31.81\textcolor{gray}{{\scriptsize $\pm$3.63}} /~~8.90\textcolor{gray}{{\scriptsize $\pm$1.40}} & 35.38\textcolor{gray}{{\scriptsize $\pm$8.43}} /10.17\textcolor{gray}{{\scriptsize $\pm$2.30}} & 35.69\textcolor{gray}{{\scriptsize $\pm$1.65}} /11.02\textcolor{gray}{{\scriptsize $\pm$1.35}} \\
Random & & & 16.33\textcolor{gray}{{\scriptsize $\pm$1.34}} /~~3.66\textcolor{gray}{{\scriptsize $\pm$0.57}} & 31.67\textcolor{gray}{{\scriptsize $\pm$3.23}} /~~7.51\textcolor{gray}{{\scriptsize $\pm$1.20}} & 32.98\textcolor{gray}{{\scriptsize $\pm$2.74}} /~~8.90\textcolor{gray}{{\scriptsize $\pm$1.23}} & 38.75\textcolor{gray}{{\scriptsize $\pm$2.49}} /10.76\textcolor{gray}{{\scriptsize $\pm$0.97}} \\\hline
PTL & \multirow{2}{*}{HERIDAL} & \multirow{2}{*}{14.64\textcolor{gray}{{\scriptsize $\pm$6.04}} /~~4.59\textcolor{gray}{{\scriptsize $\pm$1.47}}} & 25.14\textcolor{gray}{{\scriptsize $\pm$9.32}} /~~8.23\textcolor{gray}{{\scriptsize $\pm$2.54}} & 35.00\textcolor{gray}{{\scriptsize $\pm$6.30}} /12.15\textcolor{gray}{{\scriptsize $\pm$1.58}} & 37.31\textcolor{gray}{{\scriptsize $\pm$4.15}} /13.38\textcolor{gray}{{\scriptsize $\pm$0.73}} & 38.54\textcolor{gray}{{\scriptsize $\pm$7.75}} /13.37\textcolor{gray}{{\scriptsize $\pm$2.36}} \\
Random & & & 23.77\textcolor{gray}{{\scriptsize $\pm$7.78}} /~~7.43\textcolor{gray}{{\scriptsize $\pm$2.13}} & 34.28\textcolor{gray}{{\scriptsize $\pm$7.17}} /11.83\textcolor{gray}{{\scriptsize $\pm$2.37}} & 35.89\textcolor{gray}{{\scriptsize $\pm$4.74}} /12.69\textcolor{gray}{{\scriptsize $\pm$1.33}} & 40.59\textcolor{gray}{{\scriptsize $\pm$5.17}} /14.18\textcolor{gray}{{\scriptsize $\pm$2.50}} \\\hline
PTL & \multirow{2}{*}{SARD} & \multirow{2}{*}{18.27\textcolor{gray}{{\scriptsize $\pm$1.25}} /~~5.42\textcolor{gray}{{\scriptsize $\pm$0.50}}} & 31.16\textcolor{gray}{{\scriptsize $\pm$5.12}} /~~9.58\textcolor{gray}{{\scriptsize $\pm$1.86}} & 42.93\textcolor{gray}{{\scriptsize $\pm$2.58}} /13.98\textcolor{gray}{{\scriptsize $\pm$1.20}} & 46.04\textcolor{gray}{{\scriptsize $\pm$2.30}} /15.58\textcolor{gray}{{\scriptsize $\pm$0.73}} & 48.15\textcolor{gray}{{\scriptsize $\pm$1.18}} /17.05\textcolor{gray}{{\scriptsize $\pm$0.87}} \\
Random & & & 30.55\textcolor{gray}{{\scriptsize $\pm$2.77}} /~~9.37\textcolor{gray}{{\scriptsize $\pm$0.68}} & 40.69\textcolor{gray}{{\scriptsize $\pm$0.34}} /13.13\textcolor{gray}{{\scriptsize $\pm$0.12}} & 44.10\textcolor{gray}{{\scriptsize $\pm$3.84}} /14.74\textcolor{gray}{{\scriptsize $\pm$1.62}} & 45.62\textcolor{gray}{{\scriptsize $\pm$5.05}} /15.13\textcolor{gray}{{\scriptsize $\pm$2.15}} \\
\end{tabular}
}
\end{subtable}
\\\\\\
\begin{subtable}[b]{\linewidth}
\captionsetup{type=table}
\caption{Vis-200}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|rrrrr}
& & \multicolumn{5}{c}{\# of synthetic image} \\
\multicolumn{1}{c|}{method} & test set & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{2000} \\\hline
PTL & \multirow{2}{*}{VisDrone} & \multirow{2}{*}{10.55\textcolor{gray}{{\scriptsize $\pm$1.41}} /~~3.18\textcolor{gray}{{\scriptsize $\pm$0.55}}} & 11.65\textcolor{gray}{{\scriptsize $\pm$0.87}} /~~3.55\textcolor{gray}{{\scriptsize $\pm$0.35}} & 12.74\textcolor{gray}{{\scriptsize $\pm$0.90}} /~~3.99\textcolor{gray}{{\scriptsize $\pm$0.35}} & 12.96\textcolor{gray}{{\scriptsize $\pm$0.68}} /~~4.16\textcolor{gray}{{\scriptsize $\pm$0.43}} & 12.78\textcolor{gray}{{\scriptsize $\pm$0.48}} /~~4.10\textcolor{gray}{{\scriptsize $\pm$0.28}} \\
Random & & & 11.35\textcolor{gray}{{\scriptsize $\pm$1.23}} /~~3.42\textcolor{gray}{{\scriptsize $\pm$0.52}} & 12.07\textcolor{gray}{{\scriptsize $\pm$1.11}} /~~3.72\textcolor{gray}{{\scriptsize $\pm$0.46}} & 12.63\textcolor{gray}{{\scriptsize $\pm$0.59}} /~~3.95\textcolor{gray}{{\scriptsize $\pm$0.36}} & 12.59\textcolor{gray}{{\scriptsize $\pm$1.17}} /~~3.97\textcolor{gray}{{\scriptsize $\pm$0.49}} \\\hline
PTL & \multirow{2}{*}{Okutama} & \multirow{2}{*}{38.58\textcolor{gray}{{\scriptsize $\pm$4.81}} /10.25\textcolor{gray}{{\scriptsize $\pm$1.66}}} & 40.23\textcolor{gray}{{\scriptsize $\pm$2.20}} /10.71\textcolor{gray}{{\scriptsize $\pm$1.12}} & 45.56\textcolor{gray}{{\scriptsize $\pm$0.44}} /12.44\textcolor{gray}{{\scriptsize $\pm$0.51}} & 47.79\textcolor{gray}{{\scriptsize $\pm$2.47}} /12.99\textcolor{gray}{{\scriptsize $\pm$0.39}} & 46.62\textcolor{gray}{{\scriptsize $\pm$0.93}} /12.37\textcolor{gray}{{\scriptsize $\pm$0.21}} \\
Random & & & 39.99\textcolor{gray}{{\scriptsize $\pm$2.82}} /10.43\textcolor{gray}{{\scriptsize $\pm$0.48}} & 39.95\textcolor{gray}{{\scriptsize $\pm$2.33}} /10.50\textcolor{gray}{{\scriptsize $\pm$0.71}} & 41.88\textcolor{gray}{{\scriptsize $\pm$1.66}} /11.02\textcolor{gray}{{\scriptsize $\pm$0.74}} & 41.20\textcolor{gray}{{\scriptsize $\pm$0.92}} /10.55\textcolor{gray}{{\scriptsize $\pm$0.03}} \\\hline
PTL & \multirow{2}{*}{ICG} & \multirow{2}{*}{6.50\textcolor{gray}{{\scriptsize $\pm$3.17}} /~~1.39\textcolor{gray}{{\scriptsize $\pm$0.63}}} & 9.50\textcolor{gray}{{\scriptsize $\pm$1.65}} /~~2.22\textcolor{gray}{{\scriptsize $\pm$0.44}} & 20.56\textcolor{gray}{{\scriptsize $\pm$2.32}} /~~5.01\textcolor{gray}{{\scriptsize $\pm$0.40}} & 25.67\textcolor{gray}{{\scriptsize $\pm$4.82}} /~~6.44\textcolor{gray}{{\scriptsize $\pm$1.65}} & 30.48\textcolor{gray}{{\scriptsize $\pm$0.34}} /~~8.21\textcolor{gray}{{\scriptsize $\pm$0.43}} \\
Random & & & 9.27\textcolor{gray}{{\scriptsize $\pm$2.16}} /~~2.49\textcolor{gray}{{\scriptsize $\pm$0.16}} & 18.29\textcolor{gray}{{\scriptsize $\pm$5.19}} /~~4.45\textcolor{gray}{{\scriptsize $\pm$1.31}} & 23.29\textcolor{gray}{{\scriptsize $\pm$5.46}} /~~5.98\textcolor{gray}{{\scriptsize $\pm$1.31}} & 27.29\textcolor{gray}{{\scriptsize $\pm$4.52}} /~~7.41\textcolor{gray}{{\scriptsize $\pm$1.46}} \\\hline
PTL & \multirow{2}{*}{HERIDAL} & \multirow{2}{*}{14.76\textcolor{gray}{{\scriptsize $\pm$9.76}} /~~4.68\textcolor{gray}{{\scriptsize $\pm$2.72}}} & 19.87\textcolor{gray}{{\scriptsize $\pm$3.79}} /~~6.34\textcolor{gray}{{\scriptsize $\pm$0.69}} & 30.51\textcolor{gray}{{\scriptsize $\pm$6.31}} /10.34\textcolor{gray}{{\scriptsize $\pm$1.39}} & 34.76\textcolor{gray}{{\scriptsize $\pm$8.89}} /12.21\textcolor{gray}{{\scriptsize $\pm$2.76}} & 37.60\textcolor{gray}{{\scriptsize $\pm$2.12}} /13.74\textcolor{gray}{{\scriptsize $\pm$1.46}} \\
Random & & & 17.66\textcolor{gray}{{\scriptsize $\pm$7.26}} /~~5.72\textcolor{gray}{{\scriptsize $\pm$2.29}} & 26.26\textcolor{gray}{{\scriptsize $\pm$9.95}} /~~8.55\textcolor{gray}{{\scriptsize $\pm$3.30}} & 29.62\textcolor{gray}{{\scriptsize $\pm$6.13}} /10.09\textcolor{gray}{{\scriptsize $\pm$1.44}} & 33.74\textcolor{gray}{{\scriptsize $\pm$8.06}} /11.69\textcolor{gray}{{\scriptsize $\pm$2.56}} \\\hline
PTL & \multirow{2}{*}{SARD} & \multirow{2}{*}{21.87\textcolor{gray}{{\scriptsize $\pm$7.48}} /~~6.98\textcolor{gray}{{\scriptsize $\pm$1.97}}} & 30.17\textcolor{gray}{{\scriptsize $\pm$4.28}} /~~9.67\textcolor{gray}{{\scriptsize $\pm$1.03}} & 40.01\textcolor{gray}{{\scriptsize $\pm$2.13}} /13.35\textcolor{gray}{{\scriptsize $\pm$0.57}} & 46.91\textcolor{gray}{{\scriptsize $\pm$5.03}} /16.13\textcolor{gray}{{\scriptsize $\pm$1.69}} & 49.60\textcolor{gray}{{\scriptsize $\pm$1.35}} /17.73\textcolor{gray}{{\scriptsize $\pm$0.49}} \\
Random & & & 27.51\textcolor{gray}{{\scriptsize $\pm$5.72}} /~~8.74\textcolor{gray}{{\scriptsize $\pm$1.69}} & 38.96\textcolor{gray}{{\scriptsize $\pm$5.45}} /12.43\textcolor{gray}{{\scriptsize $\pm$2.31}} & 44.59\textcolor{gray}{{\scriptsize $\pm$1.56}} /14.80\textcolor{gray}{{\scriptsize $\pm$0.82}} & 43.25\textcolor{gray}{{\scriptsize $\pm$5.80}} /14.85\textcolor{gray}{{\scriptsize $\pm$2.10}} \\
\end{tabular}
}
\end{subtable}
\end{table*}

==> Tables/time_breakdown_twocolumn.tex <==
\begin{table*}[t]
\caption{{\bf \textit{Wall-clock} Training time breakdown} for sim2real transformer training and detector training. Training time is shown in \textit{mins}. The numbers in the parentheses indicate training epochs and iterations for the corresponding PTL iteration for sim2real transformer training and detector training, respectively.}
\label{tab:time_breakdown}
\begin{subtable}[b]{.46\linewidth}
\captionsetup{type=table}
\caption{sim2real transformer, Vis-20}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|rrrrr}
from-prev-iter & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} \\\hline
& 28 (100) & ~~41 (100) & ~~56 (100) & ~~69 (100) & ~~83 (100) \\
\textcolor{red}{\checkmark} & 28 (100) & 8~~~(20) & 12~~~(20) & 14~~~(20) & 17~~~(20) \\
\end{tabular}
}
\end{subtable}
&
\begin{subtable}[b]{.54\linewidth}
\captionsetup{type=table}
\caption{detector, Vis-20}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|cccccc}
from-prev-iter & 0 & 1 & 2 & 3 & 4 & 5 \\\hline
& 40 (6.0k) & 36 (6.0k) & 32 (6.0k) & 28 (6.0k) & 25 (6.0k) & 22 (6.0k) \\
\textcolor{red}{\checkmark} & 40 (6.0k) & 24 (1.2k) & 21 (1.2k) & 19 (1.2k) & 17 (1.2k) & 15 (1.2k) \\
\end{tabular}
}
\end{subtable}
\\
\begin{subtable}[b]{.46\linewidth}
\captionsetup{type=table}
\caption{sim2real transformer, Vis-50}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|rrrrr}
from-prev-iter & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} \\\hline
& 87 (100) & 101 (100) & 114 (100) & 128 (100) & 142 (100) \\
\textcolor{red}{\checkmark} & 87 (100) & 20~~~(20) & 23~~~(20) & 26~~~(20) & 29~~~(20) \\
\end{tabular}
}
\end{subtable}
&
\begin{subtable}[b]{.54\linewidth}
\captionsetup{type=table}
\caption{detector, Vis-50}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|cccccc}
from-prev-iter & 0 & 1 & 2 & 3 & 4 & 5 \\\hline
& 40 (6.0k) & 38 (6.0k) & 36 (6.0k) & 35 (6.0k) & 33 (6.0k) & 31 (6.0k) \\
\textcolor{red}{\checkmark} & 40 (6.0k) & 25 (1.2k) & 24 (1.2k) & 23 (1.2k) & 22 (1.2k) & 21 (1.2k) \\
\end{tabular}
}
\end{subtable}
\end{table*}

==> Tables/time_reduction.tex <==
\begin{table}[t]
\caption{{\bf Training time curtailment via `tuning-from-previous-iteration' strategy.} $f_t$ and $f_d$ represent the sim2real transformer and the detector, respectively. The training time is measured with wall-clock time in hours and the accuracy is indicated by MS COCO style AP@.5 and AP@[.5:.95]. The number in parentheses in `time' indicates the relative time compared to the original PTL training.}
\label{tab:time_reduction}
\centering
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{5.0pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|l|ccc|l|ccc}
& \multicolumn{4}{c|}{Vis-20} & \multicolumn{4}{c}{Vis-50} \\
from-prev-iter & \multicolumn{1}{c|}{time} & VisDrone & Okutama & ICG & \multicolumn{1}{c|}{time} & Vis & Oku & ICG \\\hline
\textcolor{gray}{Original} & ~\textcolor{gray}{10} & \textcolor{gray}{6.83/1.94} & \textcolor{gray}{30.72/7.45} & \textcolor{gray}{26.86/7.22} & ~\textcolor{gray}{16} & \textcolor{gray}{9.09/2.85} & \textcolor{gray}{42.39/11.46} & \textcolor{gray}{29.26/7.27} \\
$f_{t}$ & 6.5 \textcolor{teal}{($\times$0.65)} & 6.37/1.95 & 29.72/7.01 & 33.57/8.93 & ~~~9 \textcolor{teal}{($\times$0.56)} & 9.52/2.78 & 42.76/11.52 & 37.38/9.90 \\
$f_t$ \& $f_d$ & 5.5 \textcolor{teal}{($\times$0.55)} & 5.66/1.61 & 25.78/6.03 & 20.36/4.71 & 7.5 \textcolor{teal}{($\times$0.47)} & 7.98/2.43 & 37.14/~~9.81 & 29.50/6.78 \\
\end{tabular}
}
\end{table}
